Detecting single-trial EEG evoked potential using a wavelet domain linear mixed model: application to error potentials classification

Objective. The main goal of this work is to develop a model for multi-sensor signals such as MEG or EEG signals, that accounts for the inter-trial variability, suitable for corresponding binary classification problems. An important constraint is that the model be simple enough to handle small size and unbalanced datasets, as often encountered in BCI type experiments. Approach. The method involves linear mixed effects statistical model, wavelet transform and spatial filtering, and aims at the characterization of localized discriminant features in multi-sensor signals. After discrete wavelet transform and spatial filtering, a projection onto the relevant wavelet and spatial channels subspaces is used for dimension reduction. The projected signals are then decomposed as the sum of a signal of interest (i.e. discriminant) and background noise, using a very simple Gaussian linear mixed model. Main results. Thanks to the simplicity of the model, the corresponding parameter estimation problem is simplified. Robust estimates of class-covariance matrices are obtained from small sample sizes and an effective Bayes plug-in classifier is derived. The approach is applied to the detection of error potentials in multichannel EEG data, in a very unbalanced situation (detection of rare events). Classification results prove the relevance of the proposed approach in such a context. Significance. The combination of linear mixed model, wavelet transform and spatial filtering for EEG classification is, to the best of our knowledge, an original approach, which is proven to be effective. This paper improves on earlier results on similar problems, and the three main ingredients all play an important role.

==> Data_JNE.tex <==
% Data set - JNE

\section{Data}
\label{se:data}

We introduce an EEG data set that is used throughout the paper in order to illustrate the proposed methods.

We use the data set provided by C. Roger \etal and reported in a previous study \citename{Roger2010}. 
A brief description of the experiment is given in order to point out the main purpose of our work. Details on recordings and EEG data preprocessing are not exposed since they are independent of the current analysis.

%***************************
\subsection{\it Experiment and signal acquisition}
The data set includes ten subjects performing an Eriksen's flanker task. %\citep{Eriksen1974}. 
Each trial consists in the identification of a central letter (target) embedded in a set of three letters. Subjects were asked to respond to the target letter by pressing a button with either the left hand or right hand. The signal was recorded with $64$ scalp electrodes. After preprocessing (sampling to $1024$ Hz, artifacts removal), data were downsampled to $256$ Hz. 

%***************************
\subsection{\it Error/Correct trials classification}
For each subject, we considere two categories of trials: errors and correct trials. In this current application we do not take into acount the third class which corresponds to partial errors. In figure \ref{FCz_Monop_Correct_Errors}, differences on monopolar data between errors and correct trials are observable on grand averages. The main issue of this work is to achieved {\it single-trial} classification overpassing low signal-to-noise ratio problem.
\begin{figure}[h]
	\centering
		\includegraphics[width=0.4\textwidth]{../../ArticleNeuralEngin/Figures_JNE/FCz_Monop_Correct_Errors.pdf}
	\caption{\label{FCz_Monop_Correct_Errors} \small Grand averages (FCz) of the two types of trials (Error: red, correct:blue) for the monopolar data. For errors, a clear negativity is observable around $200$ ms after the EMG onset (zero of time). On correct trials, a large positive wave occured just after EMG onset, but no negativity is visible.}
\end{figure}

%***************************
\subsection{\it Data dimension} 
The selected trials were segmented into epochs of $500$ ms from $-100$ ms to $+400$ ms, were zero corresponds to the EMG onset that triggered the response. Each dataset in the training step correspond to a three-dimensions matrix. Thus, we consider $N^c$ trials in both classes $c=0$ (correct trials) and $c=1$ (errors) over $64$ electrodes and $128$ time-points. The total number of trials for errors and correct response is given in table~\ref{tab:NbTrials}. As a prior information based on all the subjects, we may assume that the erros represent $10\%$ of the total number of trials in each data set.

\begin{table}[h]
\caption{\label{tab:NbTrials}Total number of trials per participants for errors and correct responses.}
\begin{indented}
\item[]
\begin{tabular}{@{} l c c c c c c c c c c}
\br
\textbf{Participant} & A & B & C & D & E & F & G & H & I & J\\
\mr
Errors & 130 & 105 & ? & ? & ? & ? & 94 & 145 & 100 & 63 \\
Correct & 1376 & 1575 & ? & ? & ? & ? & 1844 & 1238 & 1167 & 907 \\
\br
\end{tabular}
\end{indented}
\end{table}

For an illustrative purpose throughout the paper, various results will be presented for only one participant. 

==> Results_JNE.tex <==

% RESULTATS - JNE

\section{Results}
\label{se:results}


%***************************
\subsection{Performance evaluation}

In the case of unbalanced classes, the performance evaluation has to be choosen carefully. Several previous works deal with model
evaluation in the presence of rare classes~\cite{Weiss2001,Weiss2004,Menardi2010}.
In this paper, different measures are considered in order to analyze classifiers performance in the unbalanced situation for EEG data.
In particular, we are interested in choosing class-dependent evaluations.

\begin{itemize}
\item \textbf{Confusion matrix, ROC curve and AUC}. In a binary classification situation, given a classifier and an observation, four outcomes are possible:  if the observation is positive and it is classified as positive, it is counted as a true positive (TP); if it is classified as negative, it is counted as a false negative (FN). If the instance is negative and it is classified as negative, it is counted as a
true negative (TN); if it is classified as positive, it is counted as a false positive (FP). 
For a test set composed of several observations, the $2\times 2$ confusion matrix summarizes those four outcomes as described in table \ref{tab:confMatrix}.


\begin{table}[h]
\caption{\label{tab:confMatrix}Confusion matrix of a binary classification problem.}
\begin{indented}
\item[]\begin{tabular}{@{}l l l l}
 \br
 & & \multicolumn{2}{c}{predicted} \\
 & &  0 & 1 \\
 actual & 0 & TN & FP \\
 & 1 & FN & TP \\
 \br
\end{tabular}
\end{indented}
\end{table}

From the confusion matrix, two main indicators can be defined:
\begin{itemize}
\item The True positive rate (TPR), or sensitivity:
\begin{equation}
TPR = \frac{TP}{(FP+TP)}
\end{equation}
\item The True negative rate (TNR) or specificity:
\begin{equation}
FNR = \frac{TN}{FN+TN} 
\end{equation}
\end{itemize}

The Receiver operating characteristic (ROC) curve is constructed by plotting the False Positive Rate (FPR = 1- TNR = 1 - Specificity) and the TPR for
different thresholds. Roc curve is one of the most frequently used tools for evaluating the accuracy of a classifier in the
presence of unbalanced classes as a trade-off between minimizing FPR and maximizing TPR can be done varying the classification threshold.

The classifier performs as better the larger the area underlying the curve (AUC) is.

\item \textbf{Good classification rate.} In the particular case of unbalanced data, the good classification rate may be calculated
for each class independently. Indeed, a common good classification rate may leads to misleading results. For example, in our problem, where the errors only represent $10\%$ of the data, the naive classification strategy of allocating all the testing data to the prevalent class would achieve a good classification rate of $90\%$. However the classifier is obviously irrelevant for detecting the errors.

\item \textbf{Pierce Skill Score.} A synthetic measurement to evaluate the quality of a previsional model, based on the
confusion matrix:
\begin{equation}
\label{eq:PSS}
PSS = H - F \,,
\end{equation}
where $H = TP/(FP+TP)$ is the good prevision rate  and $F = FP/(TN+FP)$ is the false alarm rate, such that $PSS\in \left[ -1;+1 \right]$. The closer the PSS is to $+1$, the better the classifier is for the detection of  \textit{rare} events. 
\end{itemize}


%***************************
\subsection{$N1 \neq N2$}
To analyze classifiers performance in the unbalanced case, the following setting is employed. 
A varying number of unbalanced training samples is used, based on the \textit{a priori} $10\%$ of \textit{errors}.
For each subject, the data are splitted into to distinct parts: the training samples and the test samples.
For each unbalanced training set ($\{N_1=10, \ N_2=100\} \, \{N_1=20, \ N_2=200\} \ldots \{N_1=90, \ N_2=900\}$) randomly drawn, the test set is 
composed of all the remaining data and $100$ iterations of a cross-validation are performed.

\begin{itemize}

\item Good classification rate

\begin{figure}[h]
	\centering
		\includegraphics[width=1\textwidth]{../../ArticleNeuralEngin/Figures_JNE/ResultatsBC_ErrPC.pdf}
	\caption{\emph{Participant A}: Good classification rate for an unbalanced scenario ($10\%$ error trials) and a varying number of training samples (Error-Correct). Results are given for Error test trials (left) and Correct test trials (right) and for three different classifiers. Results corresponds to the averaged good classification rate over $100$ iterations for each training sample sizes and upper and lower bar corresponds to the standard deviation.}
	\label{fig:ResultatSuj1}
\end{figure}

\item AUC. \emph{Participant A}. Averaged AUC and associated standard deviation calculated over $100$ iterations for each training samples sizes (Error-Correct). 
\begin{table}[h]
\centering
\begin{tabular}{c|c|c|c}
\hline
 $\#$ Training samples & LMM & PseudoInv LDA & Shrink LDA \\
 \hline
 \hline
 10-100 & 0.8765 (0.0331) & 0.6704 (0.0609) & 0.8635 (0.0328) \\
 20-200 & 0.9237 (0.0173) & 0.8403 (0.0386) & 0.8991 (0.0216) \\
 30-300 & 0.9384 (0.0115) & 0.8882 (0.0200) & 0.9129 (0.0145) \\
 40-400 & 0.9429 (0.0102) & 0.9087 (0.0136) & 0.9236 (0.0106) \\
 50-500 & 0.9456 (0.0113) & 0.9249 (0.0127) & 0.9341 (0.0109) \\
 60-600 & 0.9478 (0.0105) & 0.9322 (0.0133) & 0.9386 (0.0120) \\
 70-700 & 0.9482 (0.0122) & 0.9366 (0.0145) & 0.9428 (0.0128) \\
 80-800 & 0.9476 (0.0139) & 0.9370 (0.0162) & 0.9422 (0.0145) \\
 90-900 & 0.9485 (0.0159) & 0.9405 (0.0169) & 0.9451 (0.0155) \\
 \hline

\end{tabular}
\end{table}
\end{itemize}
